Long Story Short: a Summarize-then-Search Method for Long Video Question Answering

Large language models such as GPT-3 have demonstrated an impressive capability to adapt to new tasks without requiring task-specific training data. This capability has been particularly effective in settings such as narrative question answering, where the diversity of tasks is immense, but the available supervision data is small. In this work, we investigate if such language models can extend their zero-shot reasoning abilities to long multimodal narratives in multimedia content such as drama, movies, and animation, where the story plays an essential role. We propose Long Story Short, a framework for narrative video QA that first summarizes the narrative of the video to a short plot and then searches parts of the video relevant to the question. We also propose to enhance visual matching with CLIPCheck. Our model outperforms state-of-the-art supervised models by a large margin, highlighting the potential of zero-shot QA for long videos.

==> acl/sections/00-abstract.tex <==
%Large language models such as GPT-3 have demonstrated an impressive capability to adapt to new tasks without requiring task-specific training data. This capability has been particularly effective in settings such as narrative question answering, where the diversity of tasks is immense but the available supervision data is small. However, it is yet to be seen if GPT-3 can extend its zero-shot reasoning abilities to multimodal narratives.

Large language models such as GPT-3 have demonstrated an impressive capability to adapt to new tasks without requiring task-specific training data. This capability has been particularly effective in settings such as narrative question answering, where the diversity of tasks is immense, but the available supervision data is small. In this work, we investigate if such language models can extend their zero-shot reasoning abilities to long multimodal narratives in multimedia content such as drama, movies, and animation, where the story plays an essential role. We propose \modelnamelong, a framework for narrative video QA that first summarizes the narrative of the video to a short plot and then searches parts of the video relevant to the question. We also propose to enhance visual matching with \checkmodelname. Our model outperforms state-of-the-art supervised models by a large margin, highlighting the potential of zero-shot QA for long videos.

==> acl/sections/01-intro.tex <==
\section{Introduction}
\label{sec:intro}


%------------------------------------------------------------------------------
% Figure 1: Key Idea
\begin{figure*}[t]
\centering
\includegraphics[trim=0.0cm 0.45cm 0cm 0.0cm,clip,width=0.98\textwidth]{graphics/keyidea_twocolumn.pdf}
\caption{\modelnamelong (\modelname) uses Large Language Models (LLMs) (\ie GPT-3) to generate (a) Screenplay and summarized (b) Plots from video. Further details about data processing can be found in Section~\ref{sec:method}. When \modelname answer questions about the video, the model (c) validate given raw video footage with Visual Language Model, CLIP, and (d) search further grounded scripts in a backward manner, which we call \checkmodelname in Section~\ref{sec:visual-checking}.
}
\label{fig:script_idea}
\end{figure*}
%------------------------------------------------------------------------------

% Zero-shot learning challenges machine learning models to make inferences for novel tasks not explicitly seen at training time.
% Recently, large, pretrained transformer-based models like GPT-3 \cite{brown2020gpt3} have achieved impressive zero-shot capabilities for a diverse set of language generation and reasoning tasks.
% However, models like GPT-3 only accept textual prompts as input.

Recent video QA models face challenges in handling long video narrative QA tasks~\cite{choi2020dramaqa,tapaswi2016movieqa,kim2017deepstory} (\ie films, dramas, and YouTube web videos) due to the limitation in data and annotations.
This results in an inability to comprehend the long video narratives beyond answering mainly visual questions on short video clip~\cite{xu2017video,lei2018tvqa,lei2019tvqa}. 
The sizes of such long video QAs are insufficient to train the models to fully comprehend the complex narrative structures within a video, yielding sub-optimal performances.
\citep{jasani2019we} demonstrate that the supervised models rely more on language biases in the question than the narrative context:
they can obtain similar performance even without seeing any video context.
% Even their basic model which takes only question without any video context performs on par with best models which exploits full video context.
This highlights the necessity of multimodal reasoning capability beyond
small task-specific supervision.
%what model learn from scratch with the human-annotated video narrative QA datasets.


To address the challenge caused by low generalization, a zero-shot approach using pretrained Large Language Models (LLMs) can be an efficient alternative for tackling complex QA tasks~\cite{yang2021empirical}, and text context summarization~\cite{zhang2020pegasus,He2022ZCodeAP}. 
Yet, is the narrative QA capability of such LLMs transferable to the video domain?

% In this work, we explore
% %seek to answer the question of 
% whether the narrative QA capabilities of LLMs can be transferred to the video domain. We resort to a summarize-then-search approach, which has proven to be effective for tasks such as question answering and summarization in the video domain, where the challenge lies in the wide variety of tasks and the limited availability of training data. 

We propose \modelnamelong (\modelname), illustrated in figure~\ref{fig:script_idea},
that translates video clips into text screenplay format inspired by Socratic Model~\cite{zeng2022socratic}.
Using GPT-3~\cite{brown2020gpt3}, we first summarize the long video into a list of plots and then navigate both the generated summary and the raw video context
%(including Speech and Automated captions)
to resolve the given question.
Our zero-shot method shows better results than state-of-the-art supervised methods in
MovieQA and DramaQA dataset.
%the best published papers on the leaderboard that are supervised.
Furthermore, we propose \checkmodelname, a visual-text matching method to enhance visual alignment of the reasoning results provided by GPT-3. 
To summarize, our main contributions are three-fold:
\begin{enumerate}
  % \item We present synopsis generation for converting long videos as narrative summaries.
  \item We present \modelname, a framework that summarizes a long video narrative to a list of plots and retrieves the subplot relevant to the question.
  % \item We propose a new prompt search method that can allow GPT-3 to process these lengthy narratives by navigating the hierarchical context of the movie.
  \item We demonstrate the importance of considering visual alignment strength via CLIP-based matching in visual prompting.
  \item Our zero-shot approach achieves state-of-the-art performance in MovieQA~\cite{tapaswi2016movieqa}
  %, PororoQA~\cite{kim2017deepstory}
  and DramaQA~\cite{choi2020dramaqa}, outperforming supervised baselines.
\end{enumerate}

%Our approach combines scriptic knowledge with a retrieval module to access relevant portions of the detailed video context, allowing it to answer free-formed questions about a long video without the need for finetuning a target video dataset.

%We envision a long video represented by script knowledge that can explain scenes and spoken language, which could make large language model accessible without extra training on such long video.










==> acl/sections/ax-language_model_backbones.tex <==
\clearpage
\section{Language Model Backbones}
\label{sec:ax_language_model_backbones}
%------------------------------------------------------------------------------
% Figure 5: Qual examples on zero-shot audio task
\begin{figure}[h]
\centering
\includegraphics[trim=0.0cm 0.0cm 0cm 0.0cm,clip,width=0.5\textwidth]{graphics/dataset_UI.pdf}
\caption{Annotation interface of \datasetname.}

\label{fig:dataset_ui}
\end{figure}
%------------------------------------------------------------------------------
\paragraph{\modelname-Free.}
We use GPT-2-base~\cite{radford2019language} as the language model backbone for all experiments.
Since GPT-2 does not have a special start-of-sentence token,
we provide a random single token as an initial text prompt to start generation on.
This initial token is sampled from GPT-2 vocabulary with sampling weight computed with token frequency.

\paragraph{\modelname-Style.}
As summarized in Section~\ref{sec:style_ptuning}, we finetune GPT-2
on text-only corpus with style prompts to prepare the style generator backbones.
The style prompts and corresponding text corpus sources include:

\begin{itemize}
    \item \texttt{caption:} COCO Caption~\cite{lin2014microsoft}
    \item \texttt{social media:} \begin{itemize}
        \item Sentiment140~\cite{go2009twitter}
        \item MDID~\cite{kruk2019integrating}
        \item TweetEval~\cite{barbieri2020tweeteval}
    \end{itemize}
    \item \texttt{news:} GoodNews~\cite{biten2019good}
    \item \texttt{blog:} Blog Authorship~\cite{schler2006effects}
    \item \texttt{instruction:} WikiHow~\cite{koupaee2018wikihow}
    \item \texttt{story:} \begin{itemize}
        \item ROCStories~\cite{mostafazadeh2016corpus}
        \item TimeTravel~\cite{qin2019counterfactual}
    \end{itemize}
\end{itemize}

For visual news generation, we use different style prompt per news source
(\texttt{bbc:}, \texttt{guardian:}, \texttt{usa today:}, \texttt{washington post:})
to reflect writing style differences between media in VisualNews dataset~\cite{liu2021visualnews}.

==> acl/sections/xx-conclusion.tex <==
% \section{Limitation and Future work}
% To make a more informative script, character re-identification~\ref{} and co-reference resolution~\ref{} are prerequisite. instead of giving raw multimodal context to GPT-3, performance can be further improved through additional character recognition and co-reference resolution in long videos.
% \yj{tbu}

\section{Conclusion}

We introduced \modelnamelong, a summarize-then-search method to understand both global narrative and the relevant details for video narrative QA.
Also, we propose to post-check visual alignment with \checkmodelname.
Our zero-shot method improves supervised state-of-art approaches in MovieQA and DramaQA benchmarks.
We plan to release the code and the generated plot data to the public.

% There are two possible research directions beyond this work: first, providing visual descriptions better aligned with story with character re-identification and co-reference resolution improve input quality to GPT-3.
% Second, one can devise a more dynamic multi-hop search that combines global and local information in a hierarchical manner.


% \section{Acknowledgements}

\section{Limitations}

\label{sec:limitations}

Our study has some limitations, including:
% Several limitations of our study include:
\begin{enumerate}[leftmargin=*,topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
\item Experimenting with only data with English subtitles, The model can be further augmented in the multi-lingual aspect.;
\item Since our method employs capability of a large language model, power consumption and computation resource are greatly required.
\item Evaluating only with a single instance of LLM.
\end{enumerate}

\textbf{Potential Risk}.
Summarizing with GPT-3 carries some ethical risks related to the open-ended nature of the language model.
GPT-3 may (a) hallucinate fake facts about the content, (b) generate toxic utterances, or (c) implicitly embed social biases into the summary and the answer likelihoods.

==> acl/sections/xx-data.tex <==

% \subsection{\datasetname}
%\label{sec:data}
\paragraph{\datasetname.}
\label{sec:data}
To benchmark \modelnamewithlogo's capability to generate diverse styles of writing from the \emph{same} image, % in this regard,
we collect a novel dataset: \datasetname (\datasetlongname).
\datasetname is a benchmark for zero-shot diverse caption generation.
It comprises 4.8k captions from 1k images in the COCO Captions test set~\cite{lin2014microsoft}.
We collect five different writing styles that are frequently used, namely blog, social media, instruction, story, and news, as illustrated in Figure~\ref{fig:espdata}.
%We defer the details of our data and the corresponding collection process to Section~\ref{sec:ax_data_detail} and Section~\ref{sec:ax_data_collection} of the Appendix, respectively.




==> acl/sections/xx-experiment.tex <==

\input{graphics/tables/movieqa_small.tex}

% \input{graphics/tables/textqa.tex}
\input{graphics/tables/pororoqa.tex}

\input{graphics/tables/dramaqa_table.tex}


\section{Experiments}
\label{sec:experiments}

For all experiments, we use GPT-3~\cite{brown2020gpt3} (\texttt{text-davinci-003}) as the backbone language model.
Unless stated otherwise, we use the ground truth clip boundary to segment the videos.
All \modelname variants do not use any training data and thus are zero-shot methods.

\subsection{Evaluating \modelnamelong}

\textbf{MovieQA}~\cite{tapaswi2016movieqa} is a large-scale QA dataset sourced from 408 movies.
There are multiple sources of information in the dataset; subtitles, scripts, DVS, video clips, and plots.
We report four state-of-the-art supervised baselines; A2A~\cite{liu2019a2a}, PAMN~\cite{kim2019pamn}, UniversalQA~\cite{jasani2019we}, and DHTCN~\cite{liu2020dhtcn}.

Table~\ref{tab:movieqa} shows zero-shot \modelname improves over previous supervised approaches.
%in MovieQA dataset. %Importantly, our method achieves this performance despite its zero-shot nature. %: it does not use any prior QA data. %, unlike other supervised baselines.
Also, Ours-search shows strong performance even without the ground-truth segment index label.
\checkmodelname slightly improves the accuracy in the video split.
However, the difference is marginal since MovieQA often requires character-based grounding rather than general visual matching.
% most of the MovieQA questions cannot be solved by open-domain visual matching: they require character grounding of the visual information.
Finally, we experiment with the null hypothesis: No Context tests whether GPT-3 solves MovieQA by simply memorizing every fact. % and does not require context.
No Context performs worse than \modelname, rejecting the null hypothesis.

\textbf{PororoQA}~\cite{kim2017deepstory} is a video story QA dataset built from a cartoon series.
The supervised baseline takes the human-generated plot and the ground truth video segment index, while \modelname+Plot+Search takes neither.
%The dataset features 8,913 multiple-choice QA pairs.
% The cartoon series is divided into seasons, which further consist of individual episodes.
% As each QA is grounded on a specific episode, the supervised baseline takes human-generated plots and visual information about the episode.
% We instead formulate PororoQA into a problem with longer context:
% we do not provide the episode index nor the ground-truth plot.
% Instead, \modelname generates plot for the whole season and search the correct episode grounding.

Table~\ref{tab:pororoqa} summarizes our result on the PororoQA dataset.
When using both the ground-truth episode and plots, GPT-3 performs almost on par with the supervised baseline.
Substituting a human-generated summary with a model-generated one results in only a marginal performance drop.
Perhaps intriguingly, the search process works better when using model-generated plots.
We attribute this result to the fact that the human annotations are not designed for episode discriminability.

\subsection{Evaluating \checkmodelname}

\textbf{DramaQA}~\cite{choi2021dramaqa} is video QA dataset that focuses on story understanding.
The dataset is arranged with four levels of hierarchical difficulty, which follow the human cognitive-developmental stages.
We evaluate \modelname on the two high levels of DramaQA to test plot understanding.
% The baselines consist of CharacterAttention, a LXMERT~\cite{Tan2019LXMERTLC}-style model with character information incorporated as attention priors and \citep{kim2021aaai}, a pretrain-and-finetune approach. As far as we know, these are the latest results in level-wise DramaQA.
We report two latest baselines in level-wise DramaQA; CharacterAttention and \citep{kim2021aaai}.

We compare the effect of \checkmodelname and Caption, a prompt-based method of incorporating image frame descriptions extracted from BLIP~\cite{li2022blip} as inputs to GPT-3.
Table~\ref{tab:dramaqa} shows that \checkmodelname offers greater improvement than image descriptions. Also, while adding image captions improves \modelname, the gain disappears when used jointly with \checkmodelname.
We suspect that this is because frame captions provide similar information to \checkmodelname while being much noisier.


%\input{graphics/tables/human_eval.tex}



==> acl/sections/xx-method.tex <==



\begin{figure*} [t]
\centering
\includegraphics[width=0.95\textwidth]{graphics/model_arch_lss.pdf}
\caption{The qualitative result showing our proposed \modelnamelong (\modelname) model that generates and retrieves the index of raw video footage. When the model predicts the final answer from (i) the generated Summary and (ii) the retrieved text context, \checkmodelname validates each candidate's answers to revise the final answer for the question. %Further results can be found in the appendix.
}
\label{fig:architecture}
\end{figure*}

\section{Method}
\label{sec:method}


We describe \modelnamelong (\modelname), a prompt-based strategy that divides and conquers narrative video QA by summarizing the plot and retrieving relevant information with the plot. % exploits narrative of a long video for question answering.
Our objective is to predict the correct answer $a_{\hat{y}}$ from long video context $\mathbf{X}$. 
%$\hat{y} = \text{argmax}_{y} \text{QA} (\mathbf{X},q,y)$. 
Since language models can only accept tokens of fixed length (\eg 4096 tokens for GPT-3),
they cannot process the rich context (\eg subtitles or scene descriptions) of movies that typically spans two long hours.
%it cannot allow even only subtitles as context for a two-hour movie.

Thus, we introduce a summarize-then-search method for video question answering. We first divide the long video context into clip segments and summarize each segment into a subplot using GPT-3 to get the list of subplots $\mathbf{S}_X = \{s_1,s_2 \cdots s_n \}$.
Then, we retrieve video segments $\mathbf{X}_k= \{x_{k_1},\cdots,x_{k_m}\}$ relevant to the question with the subplot list as the input. We use both the full context of the selected segments and the global plot information to derive likelihood over the answer choices $p_\theta (a_1), \cdots, p_\theta (a_5)$.
Finally, we apply \checkmodelname, to strengthen the visual grounding of the selected answer. We provide the prompt templates in the appendix.

%devide a question as logical navigation of subquestions $\text{argmax}_{y} \text{QA}(\mathbf{X},q,y) = \text{argmax}_{y} \sum_{s\in\mathbf{S}} \mathbbm{1} \text{subQA}(s,q,y)$
%We ask consistent of 




\subsection{Plot Generation}
%We represent the video as textual descriptions, which consist of aligned subtitles and visual scene descriptions.
%The visual descriptions can be provided with the dataset or extracted using off-the-shelf image caption models.
%We first transcribe the video into such script context, which resembles a movie film script that includes descriptions of scenes and dialogue.
%

% We uniformly divide a long video into m segments, and collect each segment by k to make a total of $n = \lceil m/k \rceil$ scripts.
We use the ground-truth video partitions to segment the whole video into a set of shorter clips.
%We generate plot summary $S_X = s_{1 \cdots n}$ from raw video context. 
Each long video $\mathbf{X} = \{x_1, \cdots, x_n\}$ consists of $n$ clip segments, and each segment contains video $v_i$ and the corresponding text $t_i$ such as subtitle or ASR.
\begin{align*}
     \mathbf{X}' = \{(v_1, t_1), (v_2, t_1) \cdots (v_n, t_n)\}
\end{align*}
As \citep{yang2021empirical} transcribe image as language prompt for frozen GPT-3, we retrieve %anonymized 
DVS caption~\cite{rohrbach-arxiv-2016} and image captions with pretrained BLIP~\cite{li2022blip} for video $v_i\in \mathbf{X}$, and concatenate the aligned text $t_i$ as $n$ generated scripts as illustrated in figure~\ref{fig:script_idea}.
We compose a prompt to summarize the context of a video segment into a plot piece of up to three sentences and use GPT-3 to build the plot list aligned with the segment indices
$S_\mathbf{X} = \{s_1, \cdots, s_n\}$. 
%we prompt InstructGPT with ``\texttt{Summarize } ...''

\subsection{Narrative Search}
Given the summarized narrative and the question, we wish to retrieve the relatively short clip relevant to the question from the long video.
Language models generate open-ended text which is irregular and often noisy.
To retrieve the exact part of the video,
we drive the model to output indices of the plot rather than the text form. % themselves.

We first assign consecutive indices to
the list of summarized plot pieces $S_\mathbf{X} = \{ s_1, \cdots, s_n \} $ aligned with the clip segmentation.
Then, we prompt the language model to output the indices of the plot pieces $k =\{k_1, \cdots, k_m\}$ to lookup for.

The generated indices might still be noisy due to the open-ended nature of language models.
%We inspect the generated samples to find that they can 1. exceed the number of given plots, do not point any particular plot, and 3. repeat the content of the selected subplot rather than outputting the index. For the first two cases, we test a set of backup instructions to avoid the errors. The last case is handled with text-based distance search: 
When the model outputs an answer in text form, we use rouge-l~\cite{lin-2004-rouge} score to find plot piece candidates whose similarity with the generated sentence are above the specified threshold $\alpha \ge 0.5$.

Finally, we concatenate the plots $S_\mathbf{X}$, the visual and text representation of the selected segments ${\mathbf{X}'}_k = \{(v_{k_1}, t_{k_1}), \cdots, (v_{k_m}, t_{k_m})\}$, the question $q$, and the answer choices $A = \{a_1, \cdots, a_5\}$ to build the prompt input for question answering.
% We process this prompt with the language model of pretrained weights $\theta$ to derive the likelihood of the $i$-th answer choice.
% We use the model likelihood for the index token as the answer choice likelihood.
We process the prompt with the language model with weights $\theta$ and use the index token likelihood as the answer choice score.
\begin{align*}
    p_\theta(a_i) &= p_\theta (i | S_\mathbf{X}, \mathbf{X}_k, q, A)
\end{align*}

% Given the generated script and summarized synopsis, the GPT-3 can navigate the multi-level context in a long video via multi-hop prompting.
%script and synopsis level.

\subsection{Visual Checking}
\label{sec:visual-checking}

\begin{comment}
Socratic models~\cite{zeng2022socratic} as ours incorporate visual information as textual descriptions and insert them as additional prompts to the language model.
However, textual image descriptions have their limitations:
there is a trade-off between the length and thoroughness of such descriptions due to the token length limits.
\end{comment}
% not all details within an image are transferable to text
% and more practically, there is a trade-off between length and thoroughness of such description that not enough details are included in the prompt due to the token length limits.

For a tighter visual-text matching, we introduce \checkmodelname, a method to conjoin CLIP visual distance~\cite{radford2021learning} and the language model likelihood.
We start from the selected video segments $\mathbf{X}_k = \{x_{k_1}, \cdots, x_{k_m}\}$, answer choices $A = \{a_1, \cdots, a_5\}$, and answer likelihoods $P_\theta = \{p_\theta(a_1), \cdots, p_\theta(a_5)\}$ of GPT-3.

First, we use the CLIP image encoder to encode each frame $x_{k_{i_j}}$ of the selected segments. 
%We denote the clip-extracted feature with an upper bar. 
When $l$ is the number of frames within a segment:
\begin{align*}
    \bar{x}_{k_{i_j}} &=  CLIP_V(x_{k_{i_j}}) \\
    \bar{x}_{k_i} &= \{\bar{x}_{k_{i_1}}, \cdots, \bar{x}_{k_{i_l}}\} ,
    \bar{\mathbf{X}}_k = \{\bar{x}_{k_1}, \cdots, \bar{x}_{k_m}\}
\end{align*}

Then, we extract the CLIP text feature of each answer choice $\bar{a}_i = CLIP_L(a_i)$ and compare cosine similarity between the video input and the answers.
We select the best-matched frame for each answer to derive the cosine similarity score.
\begin{align*}
    c(a, \bar{\mathbf{X}}_k) &= \max_{i \le m, j \le l} cossim(\bar{a}, \bar{x}_{k_{i_j}})
\end{align*}

Then we apply the softmax function with temperature $\tau$ on the scores to get normalized visual likelihood over the answer candidates $P_c = \{p_c(a_1), \cdots, p_c(a_5)\}$.
Lastly, we multiply the answer likelihood from the language model $P_\theta$ with the visual likelihood $P_c$ to obtain the final likelihood. We simply select the answer with the maximum value as the model answer.

We choose to consider \checkmodelname only when the language model is not certain of its choice.
%of answer since long video QAs rely more on abstract plots than surface visual information.
Given the likelihoods of the top two answers $p_\theta (a_{h_1}), p_\theta (a_{h_2})$ from the language model, we measure the model certainty with binary entropy $E'$ of the re-normalized probability. 
We only use the combined likelihood when the binary entropy is greater than the given threshold $E' \ge 0.4$.
Otherwise, we do not apply \checkmodelname and just use the language model likelihood.
\begin{align*}
    &h_1 = \argmax_{i \le 5} p_\theta (a_i), 
    h_2 = \argmax_{j \le 5, j \ne h_1} p_\theta (a_j) \\
    %&p (h_i) = \frac{p_\theta (a_{h_i})}{\sum_{j \le 2} p_\theta (a_{h_j})} \\
    &E' = - p_\theta(a_{h_1}) \log p_\theta(a_{h_1}) - p_\theta(a_{h_2}) \log p_\theta(a_{h_2})
\end{align*}


==> acl/sections/xx-related-work.tex <==
\section{Related Work}
\label{sec:related_work}


Long video understanding is an important problem, but it has received less attention than shorter video understanding tasks such as video captioning and action recognition. There have been some attempts to address this problem, such as the Video QA task proposed by ~\cite{}, which requires a model to answer free-form questions about long videos. 


\textbf{Movie summarization}
generate shorter version of a screenplay as the task of finding an optimal graph chain of scene~\cite{Gorinski2015MovieSS}

\textbf{Long Viddeo QA}
The task of video question answering has been studied extensively in the literature. Several approaches have been proposed to address this task, including deep learning based models such as 

==> graphics/tables/audio_table.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{l|c|c|c}
        Model (GPT-2)                  & B@4  & M    & C    \\ \hline
        Audio Prompt + w2c            & 0.17 & 4.03 & 3.14 \\
        Oracle Prompt + w2c           & 0.80 & 5.34 & 7.07 \\ \hline 
%        Clip-Infer~\cite{tewel2022cvpr} & - & - & - \\\hline
        \modelnamewithlogo-Audio-Free         & 0.36 & 3.05 & 4.68 \\
        \modelnamewithlogo-Audio-Style        & \textbf{1.21} & \textbf{6.18} & \textbf{9.54} \\
    \end{tabular}
    \caption{Unpaired audio captioning experiments in AudioCaps test split.}
    \label{tab:audio_table}
\end{table}

==> graphics/tables/esp_table.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{l|c|c|c|c}
        Model         & Prompt & B@4 & M & C \\ \hline
        Text-Only  & \checkmark & 0.1 & 3.7 & 3.9 \\
        ClipCap-MLP  & \checkmark & 0.2 & 3.8 & 5.0 \\ \hline
        \modelnamewithlogo-Free & \checkmark & 0.6 & 5.7 & 12.8 \\
        \modelnamewithlogo-Style & \checkmark & \textbf{0.8} & \textbf{6.3} & \textbf{18.4}
    \end{tabular}
    \caption{Zero-Shot evaluation results on \datasetname.}
    \label{tab:esp_table}
\end{table}

==> graphics/tables/finetune_table.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{l|c|c|c|c}
        Model & Z\scriptsize{ero-shot} & B@4 & M & C \\
        \hline
        CLIPCap-MLP & & 27.4 & 22.4 & 94.4 \\
        CLIPCap-Full & & 32.2  & 27.1 & 108.4 \\
        \hline
        \modelnamewithlogo-Style & $\checkmark$ & 21.9 & 21.9 & 78.2 \\
        \modelnamewithlogo-MLP & & 31.2 & 25.4 & 103.1 \\
        % Ours-full & 32.2 & 26.7 & 107.9 \\
        % \modelname-full & 32.3 & 27.7  & 109.6  \\  % beam 5
        \modelnamewithlogo-Full & & \textbf{33.1} & \textbf{27.7}  & \textbf{111.1}  \\  % beam 3
    \end{tabular}
    \caption{Finetuning experiment in COCO Captions test split.}
    % and finetune the MLP encoder only for fair comparison.}
    \label{tab:finetune_table}
\end{table}

==> graphics/tables/human_eval.tex <==
{\renewcommand{\arraystretch}{1.1}
    \begin{table}[t!] \begin{center}
        \begin{adjustbox}{width=0.8\columnwidth}
        \begin{tabular}{lcccc}
            \toprule
            \multirow{2}{*}{Model} &   \multicolumn{2}{c}{Movie} & \multicolumn{2}{c}{Youtube} \\
                         
            & Vis & Inf   & Vis  & Inf  \\
            \midrule        
            Ours  & -- & --  & --   & --      \\ 
            Human & -- & --  & --   & --      \\             
            \bottomrule
        \end{tabular}
        \end{adjustbox}
    \caption{User study for generated synopsis as summarized narrative. We take the average of 5-point Likert-scale rating from three annotators. Vis. denotes visual relevance, Inf. informativeness. \yj{tbu}
    }
    \label{tab:humaneval}
    \end{center}\end{table}
}

==> graphics/tables/movieqa.tex <==
{\renewcommand{\arraystretch}{1.1}
    \begin{table*}[t!] \begin{center}
        \begin{adjustbox}{width=0.9\textwidth}
        \begin{tabular}{llcccc}
            \toprule
            & Model & Aligned & Video + Subtitle
            & Video Only & Subtitle Only \\
            \midrule                                                                                                                          
            % \multirow{5}{*}{\rotatebox[origin=c]{90}{{\footnotesize Baselines}}}              
            \multirow{4}{*}{\rotatebox[origin=c]{90}{{\footnotesize Supervised}}} &A2A~\cite{liu2019a2a} & $\checkmark$    & 41.66     & 40.28    & 41.05 \\
            & PAMN~\cite{kim2019pamn} & $\checkmark$    & 43.34     & 42.33   & 42.56                 \\             
            & UniversalQA~\cite{jasani2019we} & $\checkmark$    & 48.87 & 50.67  & 47.62                 \\ 
           & DHTCN~\cite{liu2020dhtcn} & $\checkmark$   & 49.60  & 47.38 & 48.43  \\

            \midrule          
            \multirow{4}{*}{\rotatebox[origin=c]{90}{{\footnotesize zeroshot}}} 
            & No Context & \xmark   & 36.36 & 34.28 & 38.07      \\ 
            & \modelname & $\checkmark$   & 53.44 & 49.83 & 56.42      \\ 
            & \modelname-Search & \xmark  & 51.24  & 49.00 & 53.09    \\ 
            & \modelname-Search+ClipCheck & \xmark  &  51.49  & 49.55 & 53.09      \\ 
            \bottomrule
        \end{tabular}
        \end{adjustbox}
    \caption{Evaluation on MovieQA validation split. The dataset provides GT alignment with 3 minutes of video clip on average: We also report Ours-search which can search the whole movie context without the GT alignment. \footnote{\url{http://movieqa.cs.toronto.edu/leaderboard}}
    }
    \label{tab:movieqa}
    \end{center}\end{table*}
}

==> graphics/tables/movieqa_backup.tex <==
{\renewcommand{\arraystretch}{1.1}
    \begin{table*}[t!] \begin{center}
        \begin{adjustbox}{width=0.9\textwidth}
        \begin{tabular}{llccccccc}
            \toprule
            & \multirow{2}{*}{Model} & \multirow{2}{*}{Aligned} &  \multicolumn{2}{c}{Video+Subtitle}   & \multicolumn{2}{c}{Video only} & \multicolumn{2}{c}{Subtitle only}\\
                         
            & & & Val & Test   & Val  & Test & Val  & Test\\
            \midrule                                                                                                                          
            % \multirow{5}{*}{\rotatebox[origin=c]{90}{{\footnotesize Baselines}}}              
            \multirow{4}{*}{\rotatebox[origin=c]{90}{{\footnotesize Supervised}}} &A2A~\cite{} & $\checkmark$    & 41.66    & 41.97  & 40.28   & --  & 41.05   & 41.65                \\                 
            & PAMN~\cite{} & $\checkmark$    & 43.34    & 42.53  & 42.33   & --  & 42.56   & --                \\             
            & UniversalQA~\cite{} & $\checkmark$    & 48.87    & 46.98  & 50.67   & --  & 47.62   & --                \\ 
           & DHTCN~\cite{} & $\checkmark$   & 49.60    & 47.46  & 47.38   & --  & 48.43   & --  \\

            \midrule          
            \multirow{3}{*}{\rotatebox[origin=c]{90}{{\footnotesize zeroshot}}} 
            & Ours & $\checkmark$   & xxxx  & 56.25 & xxxx & xxxx  & 56.42  & 52.23      \\ 
            & Ours-search & \xmark  & 51.38  & xxxx  & 49.00 & xxxx  & 53.09   & xxxx      \\ 
            & Ours-search+ClipCheck & \xmark  & -  & -  & 49.55 & xxxx  & -   & -      \\ 
            \bottomrule
        \end{tabular}
        \end{adjustbox}
    \caption{Evaluation on Movies with Video Clips mode in MovieQA, by default, the dataset provides GT alignment with 3 minutes of video clip on average; We also report Ours-search which is capable of searching the whole movie context without GT alignment. \footnote{\url{http://movieqa.cs.toronto.edu/leaderboard}}
    }
    \label{tab:movieqa}
    \end{center}\end{table*}
}

==> graphics/tables/rebuttal_clipcheck_shuffle.tex <==
\begin{table}[t!]
\begin{center}
        \begin{tabular}{llcc}
            \toprule
             Model & Aligned & V + S \\
            \midrule       
            \modelname  & 72.20 &  75.23   \\ 
            +\checkmodelname  & \textbf{75.78}  & \textbf{79.28}    \\             
            \midrule
            +\checkmodelname-Shuffle  & 71.74   & 73.87    \\
            \bottomrule
        \end{tabular}
    \caption{Visual checking results on DramaQA validation split.}
    \label{tab:rebuttal_clipcheck_shuffle}
\end{center}
\end{table}

==> graphics/tables/table_large.tex <==
{\renewcommand{\arraystretch}{1.3}
    \begin{table*}[t!] \begin{center}
        \begin{adjustbox}{width=\linewidth}
        \begin{tabular}{clcccccccccccccc}
            \toprule
            & \multirow{2}{*}{Model}                                 & \multicolumn{2}{c}{Video+Subtitle}    & \multicolumn{2}{c}{Video only}    & \multicolumn{2}{c}{Subtitle only}    & \multicolumn{2}{c}{PersonaChat}    & \multicolumn{2}{c}{\makecell{Wizard of\\Wikipedia}}   & \multicolumn{2}{c}{\makecell{Empathetic\\Dialogues}}    & \multicolumn{2}{c}{\makecell{Blended\\SkillTalk}}   \\
            % \cmidrule{3-16}
            \cmidrule(r{0.3em}){3-4} \cmidrule(r{0.3em}){5-6} \cmidrule(r{0.3em}){7-8} \cmidrule(r{0.3em}){9-10} \cmidrule(r{0.3em}){11-12} \cmidrule(r{0.3em}){13-14} \cmidrule(r{0.3em}){15-16}
            &                                       & Val & Test         & Val & Test         & Val & Test            & Val & Test         & Val & Test            & Val & Test        & Val & Test  \\
            \midrule                        
            \multirow{6}{*}{\rotatebox[origin=c]{90}{{\footnotesize Supervised Model}}}  
            & GPT-2                                 & 8.30  & 29.38      & 11.33 & 14.46    & 13.54  & 17.81      & 15.41 & 15.96   & 15.47 & 19.25    & 13.44  & 17.61     & 17.11  & 17.24  \\
            & DialoGPT                             & 8.37  & 32.01      & 11.28 & 15.06    & 12.89  & 18.51      & 13.87 & 17.37   & 15.92 & 19.17    & 12.46  & 18.05     & 15.22  & 16.89  \\
            & BART                                 & 7.92   & 33.20     & 10.43 & 15.65    & 14.09  & 18.96     & 13.89 & 17.99   & 14.96 & 19.95    & 12.00  & 19.26     & 15.33  & 17.42  \\
            & T5                                   & 7.51   & 31.53     & 7.74  & 13.42     & 13.76 & 16.68     & 12.99  & 16.30  & 14.20  & 17.92   & 11.17  & 16.63     & 13.48  & 15.71  \\
            & BlenderBot                           & 6.85    & 32.30    & 9.71    & 15.02    & 9.81    & 17.71    &  10.56   & 18.13    & 9.01    & 19.66    & 9.39    & 15.06    & 10.71    & 17.73 \\
            & PushShift Transformer                & 6.16 & 32.78    & 8.01 & 15.60     & 8.99 & 18.28     & 10.02 & 18.02    & 8.94 & 19.34     & 8.74 & 18.86    & 10.23 & 17.50  \\
                

            % & GPT-J                                & --    & --    & --    & --    & --    & --    & --   & --    & --    & --    & --    & --    & --    & -- \\
            
            \midrule
            \multirow{2}{*}{\rotatebox[origin=c]{90}{{\footnotesize PushShift}}}  
            % & \dialogueModelName (w/ Gold RoT)      & 6.16 & 32.78    & 8.01 & 15.60     & 8.99 & 18.28     & 10.02 & 18.02    & 8.94 & 19.34     & 8.74 & 18.86    & 10.23 & 17.50  \\
            & \dialogueModelName (Response only)          & 6.31 & 30.30    & 8.11 & 15.81    & 8.77 & 18.45     & 9.97  & 18.05   & 8.97 & 19.40     & 8.73 & 18.47     & 10.14 & 17.72  \\
            & \dialogueModelName (RoT \& Response)           & 6.22 & 31.13    & 8.10 & 15.80    & 8.81 & 18.42     & 9.97  & 17.63   & 9.04 & 18.94     & 8.73 & 18.54     & 10.13 & 17.67  \\
            \bottomrule
        \end{tabular}
        \end{adjustbox}
    \caption{Response generation results on \datasetName and other existing large-scale dialogue datasets (\S\ref{subsec:response_generation}). PPL denotes perplexity. \dialogueModelName comes with two variants: given a dialogue context (1) one generating both \textit{RoT and responses}, and (2) the other generating \textit{responses only}.}
    \label{tab:dialogue}
    \end{center}\end{table*}
}


==> graphics/tables/textqa.tex <==
{\renewcommand{\arraystretch}{1.1}
    \begin{table}[t!] \begin{center}
        \begin{adjustbox}{width=\columnwidth}
        \begin{tabular}{lcccc}
            \toprule
            \multirow{2}{*}{Model} &   \multicolumn{2}{c}{Wiki Plot} & \multicolumn{2}{c}{Movie Script} \\
                         
            & Val & Test   & Val  & Test  \\
            \midrule        
            SFU	  &  --    & 87.79   & --   & --                \\
            \midrule 
            Ours  & 92.28 & 91.78  & 89.72   & --      \\ 
            Ours-search  & 96.04  & 91.78  & --   & --      \\             
            \bottomrule
        \end{tabular}
        \end{adjustbox}
    \caption{Evaluation on Movies with wiki Plots and GT script. We give additional aligned context for Ours-search model. \yj{tbu}
    }
    \label{tab:textqa}
    \end{center}\end{table}
}

==> sections/ax-language_model_backbones.tex <==
\clearpage
\section{Language Model Backbones}
\label{sec:ax_language_model_backbones}
%------------------------------------------------------------------------------
% Figure 5: Qual examples on zero-shot audio task
\begin{figure}[h]
\centering
\includegraphics[trim=0.0cm 0.0cm 0cm 0.0cm,clip,width=0.5\textwidth]{graphics/dataset_UI.pdf}
\caption{Annotation interface of \datasetname.}

\label{fig:dataset_ui}
\end{figure}
%------------------------------------------------------------------------------
\paragraph{\modelname-Free.}
We use GPT-2-base~\cite{radford2019language} as the language model backbone for all experiments.
Since GPT-2 does not have a special start-of-sentence token,
we provide a random single token as an initial text prompt to start generation on.
This initial token is sampled from GPT-2 vocabulary with sampling weight computed with token frequency.

\paragraph{\modelname-Style.}
As summarized in Section~\ref{sec:style_ptuning}, we finetune GPT-2
on text-only corpus with style prompts to prepare the style generator backbones.
The style prompts and corresponding text corpus sources include:

\begin{itemize}
    \item \texttt{caption:} COCO Caption~\cite{lin2014microsoft}
    \item \texttt{social media:} \begin{itemize}
        \item Sentiment140~\cite{go2009twitter}
        \item MDID~\cite{kruk2019integrating}
        \item TweetEval~\cite{barbieri2020tweeteval}
    \end{itemize}
    \item \texttt{news:} GoodNews~\cite{biten2019good}
    \item \texttt{blog:} Blog Authorship~\cite{schler2006effects}
    \item \texttt{instruction:} WikiHow~\cite{koupaee2018wikihow}
    \item \texttt{story:} \begin{itemize}
        \item ROCStories~\cite{mostafazadeh2016corpus}
        \item TimeTravel~\cite{qin2019counterfactual}
    \end{itemize}
\end{itemize}

For visual news generation, we use different style prompt per news source
(\texttt{bbc:}, \texttt{guardian:}, \texttt{usa today:}, \texttt{washington post:})
to reflect writing style differences between media in VisualNews dataset~\cite{liu2021visualnews}.

==> sections/xx-data.tex <==

% \subsection{\datasetname}
%\label{sec:data}
\paragraph{\datasetname.}
\label{sec:data}
To benchmark \modelnamewithlogo's capability to generate diverse styles of writing from the \emph{same} image, % in this regard,
we collect a novel dataset: \datasetname (\datasetlongname).
\datasetname is a benchmark for zero-shot diverse caption generation.
It comprises 4.8k captions from 1k images in the COCO Captions test set~\cite{lin2014microsoft}.
We collect five different writing styles that are frequently used, namely blog, social media, instruction, story, and news, as illustrated in Figure~\ref{fig:espdata}.
%We defer the details of our data and the corresponding collection process to Section~\ref{sec:ax_data_detail} and Section~\ref{sec:ax_data_collection} of the Appendix, respectively.



